Gene-Metabolite Association Prediction with Interactive Knowledge Transfer Enhanced Graph for Metabolite Production

In the rapidly evolving field of metabolic engineering, the quest for efficient and precise gene target identification for metabolite production enhancement presents significant challenges. Traditional approaches, whether knowledge-based or model-based, are notably time-consuming and labor-intensive, due to the vast scale of research literature and the approximation nature of genome-scale metabolic model (GEM) simulations. Therefore, we propose a new task, Gene-Metabolite Association Prediction based on metabolic graphs, to automate the process of candidate gene discovery for a given pair of metabolite and candidate-associated genes, as well as presenting the first benchmark containing 2474 metabolites and 1947 genes of two commonly used microorganisms Saccharomyces cerevisiae (SC) and Issatchenkia orientalis (IO). This task is challenging due to the incompleteness of the metabolic graphs and the heterogeneity among distinct metabolisms. To overcome these limitations, we propose an Interactive Knowledge Transfer mechanism based on Metabolism Graph (IKT4Meta), which improves the association prediction accuracy by integrating the knowledge from different metabolism graphs. First, to build a bridge between two graphs for knowledge transfer, we utilize Pretrained Language Models (PLMs) with external knowledge of genes and metabolites to help generate inter-graph links, significantly alleviating the impact of heterogeneity. Second, we propagate intra-graph links from different metabolic graphs using inter-graph links as anchors. Finally, we conduct the gene-metabolite association prediction based on the enriched metabolism graphs, which integrate the knowledge from multiple microorganisms. Experiments on both types of organisms demonstrate that our proposed methodology outperforms baselines by up to 12.3% across various link prediction frameworks.

==> sections/intro.tex <==

% \qingyun{need to reorganize}
\IEEEPARstart{M}{etabolic} Metabolic engineering aims to transform microorganisms into efficient cell factories for producing value-added products in a cost-effective manner. It has served as a pivotal field targeting the enhancement of metabolite production through targeted genetic manipulations, offering profound potential for advancements in medicine, agriculture, and bioenergy.\cite{volkMetabolicEngineeringMethodologies2023}. 

However, due to the complex nature of metabolic mechanisms that reveal biological reactions inside microorganisms, these reactions involve the creation or consumption of metabolites, catalyzed by related enzymes, which form different pathways and further become a metabolic network.\cite{boobEnablingPathwayDesign2024}. 

The advance of structural databases such as UniProt\url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC9825514/}, BRENDA\url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC99121/}, and KEGG\url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC102409/} ect. include the gene, protein, reaction, and pathway information; and bioinformatics tools such as BLAST\url{https://pubmed.ncbi.nlm.nih.gov/2231712/}, \url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6207324/}, and, COBRA\url{https://www.nature.com/articles/s41596-018-0098-2} et. al further help researchers able to curate and construct the metabolic network and related model. These metabolic network models serve as a platform for understanding biochemical reactions, identifying missing genes, and discovering novel pathways. 

However, many models contain gaps, unknown reactions, or missing metabolic information, which hinder their potential in predictive accuracy and limit their usability.\cite{orthSystematizingGenerationMissing2010}. The current  YeastGEM 9.0.0 for \textbf{Saccharomyces cerevisiae} contains only 1162 genes \cite{zhangYeast9ConsensusYeast2023a}, while 6,617 open reading frames are supposed to encode genes in the Saccharomyces Genome Database. There are 2,476 genes still annotated as unknown to their molecular function\cite{wongSaccharomycesGenomeDatabase2023}.


Currently, the gap-filling process is one of the state-of-the-art methods for constructing genome-scale metabolic models. However, these gap-filling processes are mainly focused on identifying the gene-protein-reaction(GPR) for dead-end metabolites, making GEMs suitable for simulation. This process will require human experts to extract relevant information from the extensive research literature and include re-annotation of the whole genome to find the related GPR to fill the gap\cite{chenTeasingOutMissing2023},\cite{durotGenomescaleModelsBacterial2009}. 

There are automated gap-filling tools based either on topology or machine-learning methods to fill the existing gap of dead-end metabolites\url{https://academic.oup.com/bioinformatics/article/39/6/btad367/7190369}, \url{https://www.nature.com/articles/s41467-023-38110-7}. However, there is still a lack of a generally applicable method for the link prediction of unknown reactions, especially for non-model organisms.



To address these bottlenecks, we propose a new task, gene-metabolite association prediction, replacing the trivial and laborious literature mining and database analysis by inferring gene-metabolite association based on metabolism graphs constructed from metabolic mechanisms. 
\qingyun{add a task formulation}

However, performing gene-metabolite association prediction based on metabolism graphs has the following challenges. 
Firstly, existing metabolic graphs are incomplete, the association prediction based only on the metabolism graph structure is unreliable. 
Inspired by the knowledge fusion tasks, which transfer knowledge from well-studied objects to under-studied ones \cite{hinton2015distilling, luo2024knowla}, or integrate knowledge from multiple sources \cite{sun2023joint, sun2023makes}, we can also enrich the metabolic graphs by integrating the knowledge from both metabolism graphs. 
Nevertheless, the integration of graphs requires inter-graph links, which are a pair of nodes that are identical or highly similar, to connect two graphs for knowledge transfer. 
Due to the disparity between different microorganisms, detecting inter-graph links is difficult due to the heterogeneous structure between different metabolism graphs. 
The distinction with respect to the links between nodes, which are the association between gene and metabolite in our case, can be easily resolved once we find high-quality inter-graph links.
However, the difference between nodes in different metabolism graphs brings the challenge of inferring inter-graph links. The nodes that have no inter-graph links with the other graph are called ``bachelors''. The existence of ``bachelors'' severely hinders the discovery of inter-graph links.
% In addition, when inferring the gene-metabolite association, different from the traditional link prediction task which aims to predict one specific target entity given the source entity and the relation, our task aims to discover all possible associated genes. Given a specific metabolite for overproduction, there may be no genes, or multiple genes satisfying the requirement, instead of just one correct answer. 


